Complexity Results for MCMC derived from Quantitative Bounds

This paper considers how to obtain MCMC quantitative convergence bounds which can be translated into tight complexity bounds in high-dimensional {settings}. We propose a modified drift-and-minorization approach, which establishes generalized drift conditions defined in subsets of the state space. The subsets are called the "large sets", and are chosen to rule out some "bad" states which have poor drift property when the dimension of the state space gets large. Using the "large sets" together with a "fitted family of drift functions", a quantitative bound can be obtained which can be translated into a tight complexity bound. As a demonstration, we analyze several Gibbs samplers and obtain complexity upper bounds for the mixing time. In particular, for one example of Gibbs sampler which is related to the James--Stein estimator, we show that the number of iterations required for the Gibbs sampler to converge is constant under certain conditions on the observed data and the initial state. It is our hope that this modified drift-and-minorization approach can be employed in many other specific examples to obtain complexity bounds for high-dimensional Markov chains.

==> accepted-version/mcmc_defs.tex <==
% !TEX root =  paper.tex

\def\[#1\]{\begin{align}#1\end{align}}
\def\*[#1\]{\begin{align*}#1\end{align*}}

\newcommand{\defas}{\vcentcolon=}  % requires mathtools package
%\newcommand{\defas}{\equiv}

\def \bigO{\mathcal{O}}
\def \IG{\textbf{IG}}
\def \Normal{\mathcal{N}}

%% such that
\newcommand{\st}{\,:\,}

%% for writing  A | X ~ P(X) statements
\newcommand{\dist}{\ \sim\ }
\newcommand{\given}{\mid}
\newcommand{\distiid}{\overset{iid}{\dist}}
\newcommand{\distind}{\overset{ind}{\dist}}


\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\Rationals}{\mathbb{Q}}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\BorelSets}{\mathcal{B}}
\newcommand{\Nats}{\mathbb{N}}
\newcommand{\Ints}{\mathbb{Z}}
\newcommand{\NNInts}{\Ints_+}
\newcommand{\NNExtInts}{\overline{\Ints}_+}
\newcommand{\Cantor}{\2^\mathbb{N}}
\newcommand{\NNReals}{\Reals_+}

\newcommand{\as}{\textrm{a.s.}}

\newcommand{\epi}{\textrm{epi}}
\newcommand{\intr}{\textrm{int}}
\newcommand{\conv}{\textrm{conv}}
\newcommand{\cone}{\textrm{cone}}
\newcommand{\aff}{\textrm{aff}}
\newcommand{\dom}{\textrm{dom}}
\newcommand{\cl}{\textrm{cl}}
\newcommand{\ri}{\textrm{ri}}
\newcommand{\grad}{\nabla}
\newcommand{\imp}{\Rightarrow}
\newcommand{\downto}{\!\downarrow\!}
\newcommand{\upto}{\!\uparrow\!}

%\newcommand{\ind}{\perp\!\!\!\perp}
\newcommand{\ind}{\mathrel{\perp\mkern-9mu\perp}}
%\newcommand\ind{\protect\mathpalette{\protect\independenT}{\perp}} 
%\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern5mu{#1#2}}}

\newcommand{\AND}{\wedge}
\newcommand{\OR}{\vee}
\newcommand{\NOT}{\neg}

\newcommand{\dee}{\mathrm{d}}

\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\sign}{sign}

\DeclareMathOperator*{\newlim}{\mathrm{lim}\vphantom{\mathrm{infsup}}}
\DeclareMathOperator*{\newmin}{\mathrm{min}\vphantom{\mathrm{infsup}}}
\DeclareMathOperator*{\newmax}{\mathrm{max}\vphantom{\mathrm{infsup}}}
\DeclareMathOperator*{\newinf}{\mathrm{inf}\vphantom{\mathrm{infsup}}}
\DeclareMathOperator*{\newsup}{\mathrm{sup}\vphantom{\mathrm{infsup}}}
\renewcommand{\lim}{\newlim}
\renewcommand{\min}{\newmin}
\renewcommand{\max}{\newmax}
\renewcommand{\inf}{\newinf}
\renewcommand{\sup}{\newsup}

%\newcommand{\card}[1]{\#(#1)}
\newcommand{\PowerSet}{\mathcal{P}}

\newcommand{\Measures}{\mathcal{M}}
\newcommand{\ProbMeasures}{\mathcal{M}_1}

\renewcommand{\Pr}{\mathbb{P}}
\def\EE{\mathbb{E}}
\DeclareMathOperator*{\var}{var}

%% definition 
\newcommand{\defn}[1]{\emph{#1}}

\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\ceiling}[1]{\lceil #1 \rceil}

\def\bone{\mathbf{1}}
\def\Ind{\bone}

\newcommand{\cF}{\mathcal F}
\newcommand{\cG}{\mathcal G}

\DeclareMathOperator*{\Beta}{Beta}
\DeclareMathOperator*{\Bernoull}{Bernoulli}
\DeclareMathOperator*{\PP}{PP}
\DeclareMathOperator*{\Poisson}{Poisson}
\newcommand{\Uniform}{\textrm U (0,1)}

\newcommand{\equaldist}{\overset{d}{=}}
\newcommand{\inv}{^{-1}}

\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\event}[1]{\left \lbrace #1 \right \rbrace}
\newcommand{\tuple}[1]{\langle #1 \rangle}


\newcommand{\bspace}{\Omega}
\newcommand{\bsa}{\mathcal A}
\newcommand{\borelspace}{(\bspace,\bsa)}


\newcommand{\card}[1]{\##1}
%\newcommand{\as}{\textrm{a.s.}}
\newcommand{\iid}{i.i.d.}

%% for writing down stochastic processes
\newcommand{\gprocess}[2]{(#1)_{#2}}
\newcommand{\nprocess}[3]{\gprocess{#1_{#3}}{#3 \in #2}}
\newcommand{\process}[2]{\nprocess{#1}{#2}n}


%% not in love with these...
\newcommand{\of}[1]{\left ( #1 \right )}
\newcommand{\oof}[1]{( #1 )}
\newcommand{\ooof}[1]{\bigl ( #1 \bigr )}
\newcommand{\oooof}[1]{\Bigl ( #1 \Bigr )}
\newcommand{\ooooof}[1]{\biggl ( #1 \biggr )}
\newcommand{\oooooof}[1]{\Biggl ( #1 \Biggr )}

\newcommand{\oF}[1]{\left [ #1 \right ]}
\newcommand{\ooF}[1]{[ #1 ]}
\newcommand{\oooF}[1]{\bigl [ #1 \bigr ]}
\newcommand{\ooooF}[1]{\Bigl [ #1 \Bigr ]}
\newcommand{\oooooF}[1]{\biggl [ #1 \biggr ]}
\newcommand{\ooooooF}[1]{\Biggl [ #1 \Biggr ]}

\newcommand{\Of}[1]{\left \{ #1 \right \}}
\newcommand{\Oof}[1]{\{ #1 \}}
\newcommand{\Ooof}[1]{\bigl \{ #1 \bigr \}}
\newcommand{\Oooof}[1]{\Bigl \{ #1 \Bigr \}}
\newcommand{\Ooooof}[1]{\biggl \{ #1 \biggr \}}
\newcommand{\Oooooof}[1]{\Biggl \{ #1 \Biggr \}}


==> accepted-version/mcmc_headers.tex <==
% !TEX root =  paper.tex

\usepackage[foot]{amsaddr}
\usepackage[utf8]{inputenc} 
\usepackage{amsmath, amssymb,bm, cases, mathtools, thmtools}
\usepackage{verbatim}
\usepackage{graphicx}\graphicspath{{figures/}}
\usepackage{multicol}
\usepackage{tabularx}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{mathrsfs} 
\usepackage{url}
\usepackage{bbm}

\usepackage[%
    minnames=1,maxnames=99,maxcitenames=3,
    style=alphabetic,
    doi=false,url=false,
    firstinits=true,hyperref,natbib,backend=bibtex]{biblatex}
\renewbibmacro{in:}{%
  \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}}

\bibliography{mcmc_bib}

\usepackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=RawSienna]{hyperref}
\usepackage{hypernat}
\usepackage{datetime}

%% change up the fonts for fun.
%\usepackage[OT1]{eulervm} 
%\usepackage{palatino}

%\DeclareMathAlphabet\EuRoman{U}{eur}{m}{n}
%\SetMathAlphabet\EuRoman{bold}{U}{eur}{b}{n}
%\newcommand{\eurom}{\EuRoman}

%% hide equation numbers for unreferenced equations
%\mathtoolsset{showonlyrefs}

%% make text prettier
\usepackage{euscript,microtype}
%\DisableLigatures{encoding = *, family = * }

%% nicer way of making \ref'ences to theorems, lemmas, equations, sections, etc.
\usepackage[capitalize]{cleveref}

%% add entries for anything missing.
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{theorem}{Theorem}{Theorems}

%% grey out the equation numbers slightly
\makeatletter
\let\reftagform@=\tagform@
\def\tagform@#1{\maketag@@@{\ignorespaces\textcolor{gray}{(#1)}\unskip\@@italiccorr}}
\renewcommand{\eqref}[1]{\textup{\reftagform@{\ref{#1}}}}
\makeatother


%% standard marginalia note
%\setlength{\marginparwidth}{1.25in}

%% reshape the page to make it wider
%\usepackage[paperwidth=185.7mm,
%      paperheight=241.2mm,
%      textwidth=140mm,
%      textheight=230mm,
%      left=12mm]{geometry}
%\setlength{\marginparwidth}{27mm}

%% Monitor
%\usepackage[paperwidth=8in,paperheight=9in,textwidth=6in, textheight=8in,left=.5in]{geometry}
%\setlength{\marginparwidth}{1.5in}

%\input{commenting.tex}

%% For submission, make all render blank.
%\renewcommand{\LATER}[1]{}
%\renewcommand{\fLATER}[1]{}
%\renewcommand{\TBD}[1]{}
%\renewcommand{\fTBD}[1]{}
%\renewcommand{\PROBLEM}[1]{}
%\renewcommand{\fPROBLEM}[1]{}
%\renewcommand{\NA}[1]{#1}  %% Note, NA's pass through!


%% theorem styles
\declaretheorem[style=plain,numberwithin=section,name=Theorem]{theorem}
\declaretheorem[style=plain,sibling=theorem,name=Lemma]{lemma}
\declaretheorem[style=plain,sibling=theorem,name=Proposition]{proposition}
\declaretheorem[style=plain,sibling=theorem,name=Corollary]{corollary}

\declaretheorem[style=definition,sibling=theorem,name=Definition]{definition}
\declaretheorem[style=definition,qed=$\triangleleft$,sibling=theorem,name=Example]{example}
\declaretheorem[style=remark,qed=$\triangleleft$,sibling=theorem,name=Remark]{remark}
%\declaretheorem[style=definition,qed=$\triangleleft$,sibling=theorem]{fact}

%\numberwithin{equation}{section}
\numberwithin{theorem}{section}

\renewcommand{\appendixname}{}
%\renewcommand{\sectionname}{\S}

%% put ruler down the side for draft, and color it gray
%\usepackage{vruler}
%\setvruler[10pt][1][1][4][1][20pt][20pt][0pt][\textheight]
%\let\orgfillzeros\fillzeros 
%\def\fillzeros[#1]#2{% 
%  \begingroup 
%    \color[rgb]{0.8,0.8,0.8}% 
%    \orgfillzeros[{#1}]{#2}% 
%  \endgroup 
%}


==> accepted-version/section_approach_old.tex <==

Scaling classical MCMCs to very high dimensions can be problematic. Even though the chain is indeed geometrically ergodic for fixed $n$ and $p$, the convergence of Markov chains may still be quite slow as $p\to\infty$ and $n\to\infty$. %\citet{Rajaratnam2015} demonstrate that several specific bounds in the literature obtained by the drift-and-minorization method \cite{Rosenthal1995a} have problems when the dimension grows. 
For a Markov chain $\{X^{(i)},i=0,1,\dots\}$ on a state space $(\mathcal{X},\mathcal{B})$ with transition kernel $P(x,\cdot)$, defined by
\[
P(x,B)=\Pr(X^{(i+1)}\in B\,|\,X^{(i)}=x), \quad \forall x\in\mathcal{X}, B\in\mathcal{B}
\]
the general method of \cite{Rosenthal1995a} proceeds by establishing a \emph{drift condition}
\[\label{eq_old_drift}
\EE(f(X^{(1)})\,|\, X^{(0)}=x)\le \lambda f(x)+b, \quad \forall x\in \mathcal{X},
\]
where $f: \mathcal{X}\to \Reals^+$ is the ``drift function'', some $0<\lambda<1$ and $b<\infty$;
and an associated \emph{minorization condition}
\[
P(x,\cdot)\ge \epsilon Q(\cdot),\quad \forall x\in R,
\]
where $R:=\{x\in\mathcal{X}: f(x)\le d\}$ is called the ``small set'', and $d>2b/(1-\lambda)$, for some $\epsilon>0$ and some probability measure $Q(\cdot)$ on $\mathcal{X}$.
% This leads the minorization volume $\epsilon$ goes to zero exponentially fast as $p$ goes to infinity. As a result, the directly translated upper bound on the mixing time of the Markov chain increases exponentially fast as the dimension $p$ goes to infinity. 
However, it is observed, for example, in \cite{Rajaratnam2015,Qin2017}, that for many specific bounds obtained by drift-and-minorization method, when the dimension gets larger, the typical scenario for the drift condition of \cref{eq_old_drift}  seems to be $\lambda$ going to one, and/or $b$ getting much larger. This makes the ``size'' of the small set $R$ grows too fast, which leads to the minorization volume $\epsilon$ goes to $0$ exponentially fast. In the following, we give an intuitive explanation what makes a ``good'' drift condition in the high-dimensional setting.

\subsection{Intuitions}
It is useful to think the drift function $f(x)$ as an energy function \cite{Jones2001}. Then the drift condition in \cref{eq_old_drift} implies the chain tends to ``drift'' toward states which have ``lower energy'' in expectation. It is well-known that a ``good'' drift condition is established when both $\lambda$ and $b$ are small. Intuitively, $\lambda$ is small implies when the chain stays in a ``high-energy'' state in current iteration, it tends to ``drift'' back to ``low-energy'' states fast; $b$ is small implies when the chain stays in a ``low-energy'' state in current iteration, the chain tends to stay in a ``low-energy'' state as well in the next iteration. We give an analogue of this intuition in high-dimensional setting, a ``good'' drift condition is established when 
\begin{enumerate}
	\item $\lambda$ is small in the sense that it converges to $1$ slowly or is bounded away from $1$;
	\item $b$ is small in the sense that it grows at a slower rate than typical values of the drift function.
\end{enumerate}
Another way to understand the intuition is to think it as controlling the complexity order of the size of the ``small set'', $R=\{x\in\mathcal{X}: f(x)\le d\}$. Since $d>2b/(1-\lambda)$, if $\lambda$ converges to $1$ slowly or is bounded away from $1$ and $b$ is growing at a slower rate than typical values of $f(x)$, then the size of the ``small set'' $d$ can be chosen to have a small complexity order, which leads to the minorization volume $\epsilon$ goes to $0$ slowly or is bounded away from $0$. Next, we provide some advices on how to establish such a ``good'' drift condition in high-dimensional setting. 

First, assuming $\lambda$ is bounded away from $1$, we focus on the condition required for establishing $b$ which grows at a slower rate than typical values of $f(x)$. We illustrate the first advice by assuming $p$ is fixed and $n\to\infty$. Suppose the drift function is properly scaled so that we have $f(x)=\bigO(1)$ and we are able to select a typical fixed state $\tilde{x}$ such that $f(\tilde{x})=\Theta(1)$. In order to establish $b$ growing at a slower rate than typical values of $f(x)$, we hope $b=o(1)$.  On the other hand, taking expectation on both sides of \cref{eq_old_drift} yields $b\ge \EE_{\pi}[f(x)]/(1-\lambda)$ where $\EE_{\pi}[\cdot]$ denotes the expectation is taken over $x\sim \pi(\cdot)$. Since $\lambda$ is bounded away from $1$, we have both $b=\Omega(\EE_{\pi}[f(x)])$ and $b=o(1)$. This implies the drift function should be chosen such that 
$$\EE_{\pi}[f(x)]\to 0.$$
Therefore, in order to get a small $b$ in high-dimensional setting, the (properly scaled) drift function $f(\cdot)$ should satisfy the property that the distribution of the values of $f(x)$, where $x\sim\pi(\cdot)$, concentrates around $0$. Particularly,
if the stationary distribution $\pi(\cdot)$ concentrates to multiple modes as $n\to\infty$, then $\EE_{\pi}[f(x)]\to 0$ suggests that we should choose a drift function which ``captures'' the modes. In this paper, we use the name ``centered'' drift functions\cite{Qin2017} to denote drift functions that ``capture'' the modes of the stationary distribution $\pi(\cdot)$ a ``centered'' drift function.
Note that in the  literature, the drift functions used to establish the drift condition are usually not ``centered''. This is because in the traditional setting that $n$ and $p$ is fixed, a ``good'' drift condition is established whenever $\lambda$ and $b$ are small. The complexity orders of $\lambda$ and $b$ as functions of $n$ and/or $p$ are not essential so the property of ``capturing'' the posterior modes is not necessary for establishing a good drift condition. As a result, many existing quantitative bounds cannot be directly translated into tight complexity bounds since the size of the small set does not have a small complexity order. At the very least, one has to re-analyze the MCMC algorithms using ``centered'' drift functions. For example, several months after we uploaded this manuscript to arXiv, \citet{Qin2017} successfully analyzed the Albert and Chib's chain \cite{Albert1993} using ``centered'' drift functions. The original bounds for this model by \citet{Roy2007} cannot be directly translated into tight complexity orders. 

Next, we focus on establishing $\lambda$ that is either bounded away from $1$ or converges to $1$ slowly, assuming the drift function is already chosen to be ``centered''.
Intuitively, $\lambda$ describes the behavior of the Markov chain when its current state has a ``high energy''. $\lambda$ goes to $1$ very fast when $n$ and/or $p$ goes to infinity may suggest the existence of some ``bad'' states. A ``bad'' state is a state that has a ``high energy'', but the drift property becomes poor as $n$ and/or $p$ gets large. Therefore, once the Markov chain visits in one of these ``bad'' states, it drifts back toward to the ``small set'' slowly in high-dimensional cases. Since the  definition of drift condition in \cref{eq_old_drift} requires that the condition must hold for all $x\in\mathcal{X}$, $\lambda$ goes to $1$ very fast in the existence of ``bad'' states, and this cannot be remedied by choosing a different drift function. Recall that the ``small set'' is defined as $R=\{x\in\mathcal{X}: f(x)\le d\}$ where $d>2b/(1-\lambda)$,
the scenario $\lambda\to 1$ very fast leads to the ``small set'' too big, hence the minorization volume $\epsilon$ goes to zero very fast. From another perspective,  we should consider this is because the definition of drift condition in \cref{eq_old_drift} is too restrictive. 

Overall, we are able to establish a small $b$, in the sense that it grows at a slower rate than typical values of $f(x)$, using a ``centered'' drift function. However, we consider the main difficulty for establishing a proper $\lambda$ for a good drift condition suitable for high-dimensional setting is caused by the existence of some ``bad'' states when $n$ and/or $p$ gets large. Since the traditional drift condition defined in \cref{eq_old_drift} is restrictive, the traditional drift-and-minorization method is not flexible enough to deal with the ``bad'' states. 
In this following, we propose a modified drift-and-minorization approach using a generalized drift condition, where the drift function is defined only in a ``large set'' to rule out those ``bad'' states in high-dimensional cases. 

\subsection{New Quantitative Bound}
We propose a new quantitative bound, which is based on a generalized drift condition using a ``large set''. The main result is summarized in the following theorem.
\begin{theorem}\label{thm_new_drift}
	Let $\{X^{(k)}\}$ be a Markov chain  on a state space $(\mathcal{X},\mathcal{B})$ with a transition kernel $P(x,\cdot), \forall x\in\mathcal{X}$. Let $P^k(x,\cdot)$ be the $k$-step transition kernel and $\pi$ be the stationary distribution of the Markov chain. Suppose for a subset of $\mathcal{X}$, $R_0\in\mathcal{B}$, there exists a drift function $f: \mathcal{X}\to \Reals^{+}$ such that for some $\lambda<1$ and $b<\infty$, the generalized drift condition holds:
	\[\label{new_drift_cond}
	\begin{split}
	\EE(f(X^{(1)}))\,|\, X^{(0)}=x, X^{(1)}\in R_0)&\le\EE(f(X^{(1)}))\,|\, X^{(0)}=x)\\
	&\le \lambda f(x)+b, \quad \forall x\in R_0.
	\end{split}
	\]
	Furthermore, suppose that for a ``small set'' $R:=\{x\in\mathcal{X}: f(x)\le d\}$ where $d>2b/(1-\lambda)$, the Markov chain also satisfies a minorization condition:
	\[\label{eq_minorization}
	P(x,\cdot)\ge \epsilon Q(\cdot), \quad \forall x\in R,
	\]
	for some $\epsilon>0$, some probability measure $Q(\cdot)$ on $\mathcal{X}$. Finally, suppose the Markov chain begins with an initial distribution $\nu$ such that $\nu(R_0)=1$. Then for any $0<r<1$, we have
	\[\label{new_quant_bound}
	\begin{split}
	\|\mathcal{L}(X^{(k)})-\pi\|_{\var}
	&\le(1-\epsilon)^{rk} +\frac{(\alpha \Lambda)^{rk}\left[1+\EE_{\nu}[f(x)]+\frac{b}{1-\lambda}\right]-\alpha^{rk}}{\alpha^k-\alpha^{rk}}\\
	&\quad +k\,\pi(R_0^c)+\sum_{i=1}^k P^i (\nu,R_0^c),
	\end{split}
	\]
	where $\alpha^{-1}=\frac{1+2b+\lambda d}{1+d}$, $\Lambda=1+2(\lambda d+b)$ and $\EE_{\nu}[f(x)]$ denotes the expectation of $f(x)$ over $x\sim \nu(\cdot)$.
\end{theorem}
\begin{proof}
	See \cref{proof_thm_new_drift}.
\end{proof}	

Note that the new bound in \cref{thm_new_drift} assumes the Markov chain begins with an initial distribution $\nu$ such that $\nu(R_0)=1$. This assumption is not very restrictive since the ``large set'' ideally should include all ``good'' states. In high-dimensional setting, the Markov chain is not expected to converge fast beginning with any state (see \cref{discussion_initial_state} for discussions on initial states).

In order to verify the new drift condition of \cref{new_drift_cond}, one has to check a new inequality $\EE(f(X^{(1)}))\,|\, X^{(0)}=x, X^{(1)}\in R_0)\le\EE(f(X^{(1)}))\,|\, X^{(0)}=x)$. This implies the ``large set'' $R_0$ should be chosen such that the states in $R_0$ have ``lower energy'' on expectation. This is intuitive since we assume the ``bad'' states all have ``high energy'' and poor drift property when $n$ and/or $p$ gets large. We believe this condition is not very difficult to establish in practice. One trick is to choose $R_0$ by ruling out more states with ``high energy'' even if the states are not ``bad''. In \cref{section_Gibbs}, we demonstrate the use of this trick to select the ``large set'' $R_0$ so that $\EE(f(X^{(1)}))\,|\, X^{(0)}=x, X^{(1)}\in R_0)\le\EE(f(X^{(1)}))\,|\, X^{(0)}=x)$ can be easily verified.

The condition $\EE(f(X^{(1)}))\,|\, X^{(0)}=x, X^{(1)}\in R_0)\le \lambda f(x)+b, \forall x\in R_0$ essentially defines a traditional drift condition in \cref{eq_old_drift} for a new Markov kernel only on the ``large set'' $R_0$, which equals the \emph{conditional} transition kernel $P'(x,B):=P(x,B\cap R_0)/P(x,R_0),\forall x\in R_0, B\in \mathcal{B}$. The first two terms in the upper bound \cref{new_quant_bound} are indeed an upper bound on the total variation distance of this ``restricted'' Markov chain. Note that the general idea of studying the restriction of a Markov chain to some ``good'' subset of the state space has appeared in the literature, such as \cite{Martin2000,Dyer2003,Jerrum2004,Efthymiou2016,Mangoubi2017} and the references therein, in which different ways of restrictions have been considered for different reasons. Our condition is to assume that the chain has never left the ``large set''. The goal of considering this ``restricted'' chain is to obtain better control on the dependence on $n$ and $p$ for the upper bound.

The last two terms in the upper bound \cref{new_quant_bound} give an upper bound of the probability that the Markov chain will visit $R_0^c$ starting from either the initial distribution $\nu$ or the stationary distribution $\pi$. Therefore, the proposed method in \cref{thm_new_drift} is a generalized version of the classic drift-and-minorization method \cite{Rosenthal1995a} by allowing the drift condition is established in a chosen ``large set''. Indeed, if we choose $R_0=\mathcal{X}$, then \cref{new_quant_bound} reduces to 
\[
\begin{split}
\|\mathcal{L}(X^{(k)})-\pi\|_{\var}
&\le(1-\epsilon)^{rk} +\frac{(\alpha \Lambda)^{rk}\left[1+\EE_{\nu}(f(x))+\frac{b}{1-\lambda}\right]-\alpha^{rk}}{\alpha^k-\alpha^{rk}}.
\end{split}
\]
This bound is almost the same as \cite[Theorem 12]{Rosenthal1995a}, except slightly tighter due to the terms $\alpha^{rk}$.

One more note about \cref{new_quant_bound} is that the new bound does not decrease exponentially with $k$. For example, the term $k\,\pi(R_0^c)$ is linear increasing with $k$ for fixed $n$ and $p$. We emphasize that we do not aim to prove a Markov chain is geometrically ergodic here.  An upper bound which decreases exponentially with $k$ for fixed $n$ and $p$ does not guarantee to have a tight complexity order, which has been discussed in \cite{Rajaratnam2015}. Instead, our new bound in \cref{new_quant_bound} is designed for controlling complexity orders of $n$ and/or $p$ for high-dimensional Markov chains.

Furthermore, the Markov chain to be analyzed  in \cref{thm_new_drift} does not have to be geometrically ergodic. The proof of \cref{new_quant_bound} only implies that, after ruling out ``bad'' states, the ``restricted'' Markov chain defined in the ``large set'', using the \emph{conditional} transition kernel $P'(x,B):=P(x,B\cap R_0)/P(x,R_0),\forall x\in R_0, B\in \mathcal{B}$ is geometrically ergodic. Therefore, technically speaking, the new bound in \cref{new_quant_bound} can be used to analyze non-geometrically ergodic high-dimensional Markov chains.

\subsection{Complexity Bound} The proposed new bound in \cref{thm_new_drift} can be used to obtain complexity bounds in high-dimensional setting. The key is to balance the complexity orders of $k$ required for both the first two terms and the last two terms of the upper bound in \cref{new_quant_bound} to be small. The complexity order of $k$ for the first two terms to be small can be controlled by adjusting the ``large set''. The ``large set'' should be kept as large as possible provided that ``bad'' states have been ruled out. The complexity order of $k$ required for the last two terms to be small is determined by
\[
k\,\pi(R_0^c)+\sum_{i=1}^k P^i (\nu,R_0^c)\to 0.
\]
This may involve (carefully) bounding the tail probability of the transition kernel, depending on the definition of the ``large set'' and the complexity order aimed to establish.


In the next section, we employ the modified drift-and-minorization method to prove a certain realistic Gibbs sampler algorithm converges in $\bigO(1)$. We first choose a particular ``centered'' drift function $f(x)$ and identify the ``bad'' states. In our Gibbs sampler example, one coordinate of the state $x$ corresponds to one particular parameter of the MCMC model, and the ``bad'' states correspond to those whose value of this particular parameter is close to zero. Then we define the ``large set'' by ruling out the ``bad'' states. This allow us to obtain a quantitative bound using \cref{thm_new_drift}. Finally, under high-dimensional setting, the obtained quantitative bound can be translated into a complexity bound, which shows that the mixing time of the Gibbs sampler is $\bigO(1)$.
